Efficient List Decoding of Convolutional Polar Codes

An efficient implementation of min-sum SC/list decoding of convolutional polar codes is proposed. The complexity of the proposed implementation of SC decoding is more than two times smaller than the straightforward implementation. Moreover, the proposed list decoding algorithm does not require to copy any LLRs during decoding.

==> alg2e-Encode.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: Encode
%%%%%%%%%%%%%%%%%%%%%%%%%
\onealg{
\caption{\texttt{Encode}$(m, a_0^{k-1}, \mI)$}
\label{alg:encode}

$n \gets 2^m$, $c \gets \bnull^{n}$, $c_{\mI}\gets a_0^{k-1}$, $N \gets 2$ \label{l:subv} \\
\For{$\lambda \gets m \dots 1$}{\label{l:en-lb}
\For{$g \gets 0 \dots n/N-2$}{ \label{l:en:s1b}
\For{$j \gets 0 \dots N/2-1$}{
$i \gets gN+N/2+j$\\
$c_i \opgets c_{i+N/2}$ \label{l:en:s1e}}}
\For{$g \gets 0 \dots n/N-1$}{ \label{l:en:s2b}
\For{$j \gets 0 \dots N/2-1$}{
$i \gets gN+j$ \\
$c_{i} \opgets c_{i+N/2}$ \label{l:en:s2e}}}
$N \gets 2N$ \label{l:en-le}}
\Return{$c_{[n]}$}
}




==> alg2e-SCDecoding.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: DecodeSC
%%%%%%%%%%%%%%%%%%%%%%%%%
\IncMargin{1em}\begin{algorithm}
\caption{\texttt{DecodeSC}$(n=2^m, y_{[n]}, \mI, W)$}
\label{alg:decodesc}
allocate $\bfT[0..m]$\\
\For{$\lambda \in[m+1]$}{
    $\bfT[\lambda]\gets $ 2D array of size $2^{m-\lambda}\times8$
}
\lFor*{$i \in[n/2]$}{\label{l:decodesc-init0}
\For{$(a,b) \in \bF^2$}{$\bfT[1][i][a,b]\gets \ln \frac{W(0|y_i)W(0|y_{i+n/2})}{W(a+b|y_i)W(b|y_{i+n/2})}$}}\label{l:decodesc-init1}
\For{$\vp \gets  0 \dots n-1$}{
$l\gets $ \call{CalcT\_SC}$(\vp)$ \label{l:decodesc-ct}\\
$\bfC[m][\vp \bmod 2]\gets \mathbf 1[\vp \in \mI \;\wedge\; l < 0]$ \label{l:decodesc-hd}\\
\call{UpdateC\_SC}$(\vp)$ \label{l:decodesc-uc}
}
$\hat u_{[n]}\gets \bfC[0][0..n-1](Q^{(n)})^{-1}$ \label{l:decodesc-cw2data}\\
\Return{$\hat u_{\mI}$} \label{l:decodesc-ret}
\end{algorithm}\DecMargin{1em}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: CalcT_SC
%%%%%%%%%%%%%%%%%%%%%%%%%
\IncMargin{1em}\begin{algorithm}
\DontPrintSemicolon
\caption{\texttt{CalcT\_SC}$(\vp)$}
\label{alg:calctsc}

$n \gets  2^m$, $\vp\gets \xi$ \\
\lIf*{$\vp =n-2$}{\Return{$\Delta \mu_1^1(\bfT[m][0],\bfC[m][1])$}} \label{l:calctsc-n-2}
\If{$\vp =n-1$}{
    $a\gets \bfC[m-1][2]$, $b\gets \bfC[m][0]$\\
    \Return{$\Delta \mu_2^0\left(\bfT[m][0],a+b,b\right)$ \label{l:calctsc-n-1}} 
}
$\lambda_\text{min} \gets  m$\\
\eIf{$\vp =0$}{ \label{l:calctsc-phi00}
    \For{$\lambda \gets  2 \dots m-1$}{ 
      \For{$i \in [2^{m-\lambda}]$}{
            $\bfT[\lambda][i] \gets \sigma_{0,2,2}(\bfT[\lambda-1][i], \bfT[\lambda-1][i+2^{m-\lambda}])$ \label{l:calctsc-phi01}
        }
    }
}
{
    \While{$(\vp\equiv  1 \bmod 2) \wedge (\lambda_\text{min}>2) \wedge (\vp\neq 1)$}{ \label{l:calctsc-lmin0}
        $\vp\gets \floor{\vp/2}, \; \lambda_\text{min}\gets \lambda_\text{min}-1$ \label{l:calctsc-lmin1}
    }
}
\For{$\lambda \gets  \mu \dots m$}{ \label{l:calctsc-main0}
$\sigma\gets$ \texttt{GetClusterOp}$(\lambda,\vp)$ \label{l:calctsc-op0}\\
\For{$i \gets  0 \dots 2^{m-\lambda}-1$}{
$\bfT[\lambda][i] \gets \sigma(\bfT[\lambda-1][i]$, $\bfT[\lambda-1][i+2^{m-\lambda}], \bfC[\lambda][2i], \bfC[\lambda][2i+1])$ \label{l:calctsc-op1}
}
\lIf{$\vp\neq 0$}{$\vp \gets  2\vp+1$ \label{l:calctsc-main1}}
}
\Return{$\Delta \mu_0^2(\bfT[m][0])$}
\end{algorithm}\DecMargin{1em}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: GetClusterOp
%%%%%%%%%%%%%%%%%%%%%%%%%
\IncMargin{1em}\begin{algorithm}
\DontPrintSemicolon
\caption{\texttt{GetClusterOp}$(\lambda,\vp)$}
\label{alg:getclusterop}

\lIf*{$\vp =0$}{\Return{$\sigma_{0,3,1}$}}
\lIf*{$\vp =2^\lambda-3$}{\Return{$\sigma_{1,3,0}$}}
\lIf*{$\vp =2^\lambda-2$}{\Return{$\sigma_{2,2,0}$}}
\lIf*{$\vp \equiv 1 \bmod 2$}{\Return{$\sigma_{1,3,2}$}}
\Return{$\sigma_{2,3,1}$}
\end{algorithm}\DecMargin{1em}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: UpdateC_SC
%%%%%%%%%%%%%%%%%%%%%%%%%
\IncMargin{1em}\begin{algorithm}
\DontPrintSemicolon
\caption{\texttt{UpdateC\_SC}$(\vp)$}
\label{alg:updatecsc}

$\lambda \gets  m, \; N\gets 1$ \\
\While{$\vp \neq 0 \wedge \; \lambda \neq 0$}{ 
  $C\gets\bfC[\lambda],\;C'\gets\bfC[\lambda-1]$ \\
  $\psi \gets  \floor{\frac{\vp-1}{2}},\; b\gets \psi \bmod 2$\label{l:updatecsc-odd0}\\
  \If{$\vp \equiv 1 \bmod 2$}{ \label{l:updatecsc-com1}
    \For{$i \in[N]$}{
      \If{$\lambda = 1$}{
        $C'[i]\gets C[2i]+C[2i+1]$\\ \label{l:updatecsc-l10}
        $C'[i+N]\gets C[2i+1]$} \label{l:updatecsc-l11}
      \Else{
        $C'[2i+b]\gets C[2i]+C[2i+1]$\\
        $C'[2i+b+2N]\gets C[2i+1]$
    }
    \lIf{$\vp \neq 2^\lambda\!-\!1$}{\textbf{break}}}\label{l:updatecsc-odd1}
  }
  \Else{\label{l:updatecsc-even0}
    \For{$i \in[N]$}{  
      $C'[2i+b]\pgets C[2i]$\\
      $C'[2i+b+2N]\pgets C[2i]$ \label{l:updatecsc-even1}
    }
  }
  $\lambda \gets \lambda \!-\!1, \; \vp\gets \psi, \; N\gets 2N$ \label{l:updatecsc-com2}
}
\end{algorithm}\DecMargin{1em}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm: Sigma
%%%%%%%%%%%%%%%%%%%%%%%%%
\IncMargin{1em}\begin{algorithm}
\DontPrintSemicolon
\caption{$\sigma_{i,t,j}(A,B,x)$}
\label{alg:sigma}

\KwIn{$t'$-clusters $A$ and $B$, $2t'=i+t+j$, bit vector $u$, containing $i$ or more bits. If more than $i$ bits are provided, the bits after $u_{i-1}$ are ignored}
\KwOut{The resulting $t$-cluster $T\in\bR^{2^t}$}
$T[0..2^t-1]\gets -\infty$\\
\For{$x \in\bF^t$}{
  \For{$z \in\bF^j$}{
    $a\gets (u_{[i]}, x_{[t]}, z_{[j]})X^{(2t')}$\\ 
    $b\gets (u_{[i]}, x_{[t]}, z_{[j]})Z^{(2t')}$\\ 
    $T[x]\gets \max\set{T[x], A[a]+B[b]}$
  }
}
\Return{$T$}
\end{algorithm}\DecMargin{1em}


